Characterizing the Circumgalactic Medium of Nearby Galaxies with HST/COS and HST/STIS Absorption-Line Spectroscopy: II. Methods and Models

We present basic data and modeling for a survey of the cool, photo-ionized Circum-Galactic Medium (CGM) of low-redshift galaxies using far-UV QSO absorption line probes. This survey consists of "targeted" and "serendipitous" CGM subsamples, originally described in Stocke et al. (2013, Paper 1). The targeted subsample probes low-luminosity, late-type galaxies at $z<0.02$ with small impact parameters ($\langle\rho\rangle = 71$ kpc), and the serendipitous subsample probes higher luminosity galaxies at $z\lesssim0.2$ with larger impact parameters ($\langle\rho\rangle = 222$ kpc). HST and FUSE UV spectroscopy of the absorbers and basic data for the associated galaxies, derived from ground-based imaging and spectroscopy, are presented. We find broad agreement with the COS-Halos results, but our sample shows no evidence for changing ionization parameter or hydrogen density with distance from the CGM host galaxy, probably because the COS-Halos survey probes the CGM at smaller impact parameters. We find at least two passive galaxies with H I and metal-line absorption, confirming the intriguing COS-Halos result that galaxies sometimes have cool gas halos despite no on-going star formation. Using a new methodology for fitting H I absorption complexes, we confirm the CGM cool gas mass of Paper 1, but this value is significantly smaller than found by the COS-Halos survey. We trace much of this difference to the specific values of the low-$z$ meta-galactic ionization rate assumed. After accounting for this difference, a best-value for the CGM cool gas mass is found by combining the results of both surveys to obtain $\log{(M/M_{\odot})}=10.5\pm0.3$, or ~30% of the total baryon reservoir of an $L \geq L^*$, star-forming galaxy.

==> tab_absprop.tex <==
\begin{deluxetable*}{cllCCCl}
\tablecaption{Multi-Component Absorption Line Fits\label{tab:absprop}}
\tablewidth{0pt}
\tabletypesize{\small}
\tablehead{ \colhead{System} & \colhead{Sight Line} & \colhead{Ion} & \colhead{$cz_{\rm abs}$} & \colhead{$b$} &  \colhead{$\log{N}$} & \colhead{Comments} \\ \colhead{\#} & & & \colhead{(\kms)} & \colhead{(\kms)} & \colhead{($N$ in cm$^{-2}$)} }

\colnumbers
\startdata
  1 & 1ES~1028+511      & \HI\    &   728 &  27.3\pm 5.9 &  13.30\pm0.06 & Voigt profile fit to \lya\ \\
  2 & 1ES~1028+511      & \HI\    &   967 &  21.8\pm 2.5 &  14.30\pm0.15 & Voigt profile fit to \lya\ \\*
    &                   & \CIV\   &   954 &  12.3\pm 6.6 &  13.34\pm0.10 & Simultaneous fit to doublet \\
  3 & 1SAX~J1032.3+5051 & \HI\    &   704 &  29.6\pm13.1 &  13.08\pm0.27 & Voigt profile fit to \lya\ \\
  4 & FBQS~J1010+3003   & \HI\    &  1264 &  36.9\pm11.9 &  13.27\pm0.09 & Voigt profile fit to \lya\ \\
  5 & FBQS~J1010+3003   & \HI\    &  1380 &  36.8\pm 2.9 &  14.47\pm0.08 & Voigt profile fit to \lya\ \\
  6 & HE~0435--5304     & \HI\    &  1514 &  29.4\pm 3.7 &  13.80\pm0.04 & Voigt profile fit to \lya\ \\
  7 & HE~0435--5304     & \HI\    &  1647 &  67.5\pm15.9 &  14.00\pm0.11 & BLA; Voigt profile fit to \lya\ \\
  8 & HE~0435--5304     & \HI\    &  1719 &  25.3\pm11.8 &  13.49\pm0.30 & Voigt profile fit to \lya\ \\
  9 & HE~0439--5254     & \HI\    &  1581 &   5.6\pm14.3 &  12.76\pm0.24 & Voigt profile fit to \lya\ \\
 10 & HE~0439--5254     & \HI\    &  1653 &  30.0\pm 6.7 &  15.04\pm0.50 & Voigt profile fit to \lya\ \\*
    &                   & \CII\   &       &              & <13.76        & Upper limit from intervening line \\*
    &                   & \CIV\   &  1643 &  11.9\pm 1.7 &  13.94\pm0.07 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &              & <13.29        & Upper limit from intervening line \\*
    &                   & \SiIII\ &  1662 &  25.4\pm 5.6 &  13.05\pm0.08 & \\*
    &                   & \SiIV\  &  1642 &  17.0\pm 3.4 &  12.99\pm0.05 & Simultaneous fit to doublet \\*
    &                   & \OI\    &       &  15          & <13.63        & \\*
    &                   & \NV\    &       &  15          & <13.48        & \\*
    &                   & \FeII\  &       &  15          & <13.60        & \\
 11 & HE~0439--5254     & \HI\    &  1763 & 105.3\pm56.7 &  13.49\pm0.20 & BLA; Voigt profile fit to \lya\ \\
 12 & HE~0439--5254     & \HI\    &  1805 &  14.0\pm 5.0 &  13.27\pm0.10 & Voigt profile fit to \lya\ \\
 13 & HE~0439--5254     & \HI\    &  3861 &  35.7\pm 1.7 &  14.12\pm0.02 & Voigt profile fit to \lya\ \\
 14 & PG~0832+251       & \HI\    &  5221 &  37.3\pm 1.4 &  18.34\pm0.21 & Voigt profile fit to \lya, $cz$ fixed \\*
    &                   & \CI\    &       &  10          & <13.16        & \\*
    &                   & \CII\   &  5224 &  45.6\pm 2.1 &  15.11\pm0.06 & 1334~\AA\ line only \\*
    &                   & \CIV\   &  5189 &  10.1\pm 4.7 &  14.49\pm0.58 & Simultaneous fit to doublet \\*
    &                   & \CIV\   &  5246 &  29.8\pm 5.1 &  14.61\pm0.05 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &  5223 &  34.6\pm 1.0 &  14.49\pm0.03 & Simultaneous fit to 4 available lines \\*
    &                   & \SiIII\ &  5230 &  43.1\pm 6.4 &  14.54\pm0.30 & \\*
    &                   & \SiIV\  &  5209 &  44.2\pm 6.6 &  13.83\pm0.10 & Simultaneous fit to doublet \\*
    &                   & \SiIV\  &  5251 &  19.4\pm 4.0 &  13.63\pm0.15 & Simultaneous fit to doublet \\*
    &                   & \OI\    &  5196 &  14.4\pm 5.4 &  14.37\pm0.09 & \\*
    &                   & \OI\    &  5238 &  10.0\pm 0.0 &  14.92\pm0.21 & \\*
    &                   & \OVI\   &       &              & <14.19        & Upper limit from intervening line \\*
    &                   & \NV\    &       &  40          & <13.68        & \\*
    &                   & \FeII\  &  5199 &  12.6\pm 6.6 &  13.73\pm0.10 & Simultaneous fit to 4 available lines \\*
    &                   & \FeII\  &  5236 &   9.6\pm 3.1 &  14.14\pm0.08 & Simultaneous fit to 4 available lines \\*
    &                   & \FeIII\ &       &  10          & <14.17        & \\
 15 & PG~0832+251       & \HI\    &  5337 &  48.0:       &  14.96:       & BLA; Voigt profile fit to \lya, $cz$ fixed \\*
    &                   & \CI\    &       &  10          & <13.16        & \\*
    &                   & \CII\   &  5346 &  12.5\pm 4.5 &  13.59\pm0.07 & 1334~\AA\ line only \\*
    &                   & \CIV\   &  5327 &  20.5\pm 2.7 &  14.41\pm0.07 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &              & <12.71        & \\*
    &                   & \SiIII\ &  5346 &  30.1\pm11.0 &  12.98\pm0.14 & \\*
    &                   & \SiIV\  &  5327 &  60.4\pm43.9 &  13.24\pm0.27 & Simultaneous fit to doublet \\*
    &                   & \OI\    &       &  10          & <13.73        & \\*
    &                   & \NV\    &       &              & <13.77        & Upper limit from intervening line \\*
    &                   & \FeII\  &       &  10          & <13.65        & \\*
    &                   & \FeIII\ &       &  10          & <14.17        & \\
 16 & PG~0832+251       & \HI\    &  5396 &  26.7:       &  14.28:       & Voigt profile fit to \lya, $cz$ fixed \\*
    &                   & \CI\    &       &  10          & <13.16        & \\*
    &                   & \CII\   &  5394 &  16.4\pm11.1 &  13.27\pm0.15 & 1334~\AA\ line only \\*
    &                   & \CIV\   &  5385 &  11.1\pm 3.8 &  13.83\pm0.12 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &              & <12.71        & \\*
    &                   & \SiIII\ &  5411 &  10.0\pm 0.0 &  12.34\pm0.25 & \\*
    &                   & \SiIV\  &  5394 &  15.8\pm24.3 &  12.36\pm0.87 & Simultaneous fit to doublet \\*
    &                   & \OI\    &       &  10          & <13.73        & \\*
    &                   & \NV\    &       &  40          & <13.68        & \\*
    &                   & \FeII\  &       &  10          & <13.65        & \\*
    &                   & \FeIII\ &       &  10          & <14.17        & \\
 17 & PG~0832+251       & \HI\    &  5444 &  39.0\pm21.2 &  15.08\pm2.08 & Voigt profile fit to \lya, $cz$ fixed \\*
    &                   & \CI\    &       &  10          & <13.16        & \\*
    &                   & \CII\   &  5440 &  10.0\pm 0.0 &  13.58\pm0.07 & 1334~\AA\ line only \\*
    &                   & \CIV\   &  5437 &  32.2\pm 4.6 &  14.13\pm0.04 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &  5447 &  14.3\pm 6.0 &  12.71\pm0.09 & Simultaneous fit to 4 available lines \\*
    &                   & \SiIII\ &  5461 &  65.2\pm33.7 &  12.74\pm0.21 & \\*
    &                   & \SiIV\  &  5436 &  10.0\pm 0.0 &  12.78\pm0.09 & Simultaneous fit to doublet \\*
    &                   & \OI\    &       &  10          & <13.73        & \\*
    &                   & \NV\    &       &  40          & <13.68        & \\*
    &                   & \FeII\  &       &  10          & <13.65        & \\*
    &                   & \FeIII\ &       &  10          & <14.17        & \\
 18 & PMN~J1103--2329   & \HI\    &  1113 &  20.0\pm 0.0 &  13.15\pm0.67 & Voigt profile fit to \lya\ \\*
 19 & PMN~J1103--2329   & \HI\    &  1194 &  48.6\pm 7.0 &  14.76\pm0.16 & BLA; Voigt profile fit to \lya\ \\*
    &                   & \CI\    &       &  20          & <13.33        & \\*
    &                   & \CII\   &       &  20          & <13.22        & \\*
    &                   & \CIV\   &  1189 &  23.6\pm 1.8 &  14.27\pm0.04 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &  20          & <12.26        & \\*
    &                   & \SiIII\ &  1195 &  28.9\pm 0.5 &  12.95\pm0.01 & \\*
    &                   & \SiIV\  &  1191 &  25.1\pm 4.8 &  13.01\pm0.05 & Simultaneous fit to doublet \\*
    &                   & \NV\    &  1201 &  52.5\pm10.3 &  13.66\pm0.06 & Simultaneous fit to doublet \\*
    &                   & \FeII\  &       &  20          & <13.84        & \\
 20 & RX~J0439.6--5311  & \HI\    &  1638 &  44.4\pm30.7 &  13.87\pm0.81 & BLA; Voigt profile fit to \lya\ \\
 21 & RX~J0439.6--5311  & \HI\    &  1674 &  20.0\pm 0.0 &  15.53\pm0.43 & Voigt profile fit to \lya\ \\*
    &                   & \CI\    &       &  10          & <13.20        & \\*
    &                   & \CII\   &       &  10          & <13.11        & \\*
    &                   & \CIV\   &  1673 &  18.7\pm 4.3 &  13.55\pm0.06 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &              & <12.56        & Upper limit from intervening line \\*
    &                   & \SiIII\ &  1685 &  13.3\pm 2.7 &  12.96\pm0.07 & \\*
    &                   & \SiIV\  &  1667 &  21.6\pm 7.1 &  12.84\pm0.08 & Simultaneous fit to doublet \\*
    &                   & \OI\    &       &  10          & <13.58        & \\*
    &                   & \NV\    &       &  20          & <13.12        & \\*
    &                   & \FeII\  &       &  10          & <13.66        & \\
 22 & RX~J0439.6--5311  & \HI\    &  1734 &  20.0\pm 0.0 &  13.29\pm0.15 & Voigt profile fit to \lya\ \\
 23 & SBS~1108+560      & \HI\    &   654 &    \nodata   &    \nodata    & No \lya\ fit possible \\*
    &                   & \CI\    &       &              & <13.57        & Upper limit from intervening line \\*
    &                   & \CII\   &       &              & <16.92        & Blended with Ly-series at $z=0.4634$ \\*
    &                   & \CIV\   &   656 &  31.9\pm 2.9 &  14.53\pm0.04 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &   656 &  11.3\pm 3.9 &  16.18\pm1.50 & 1526~\AA\ line only \\*
    &                   & \SiIII\ &   643 &  22.7\pm31.2 &  13.97\pm1.88 & \\*
    &                   & \SiIV\  &   658 &  48.5\pm 2.2 &  13.96\pm0.02 & Simultaneous fit to doublet \\*
    &                   & \NV\    &       &  40          & <13.93        & \\*
    &                   & \FeII\  &   653 &  18.1\pm 3.7 &  14.41\pm0.08 & 1608~\AA\ line only \\
 24 & SBS~1108+560      & \HI\    &   715 &    \nodata   &    \nodata    & No \lya\ fit possible \\*
    &                   & \CI\    &       &  10          & <13.03        & \\*
    &                   & \CII\   &       &              & <15.67        & Blended with Ly-series at $z=0.4634$ \\*
    &                   & \CIV\   &   713 &  16.2\pm 4.2 &  14.13\pm0.08 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &   716 &   9.1\pm 3.1 &  14.12\pm0.28 & 1526~\AA\ line only \\*
    &                   & \SiIII\ &   718 &  14.9\pm15.0 &  15.83\pm2.87 & \\*
    &                   & \SiIV\  &   712 &   9.7\pm 2.8 &  13.23\pm0.08 & Simultaneous fit to doublet \\*
    &                   & \NV\    &       &  40          & <13.93        & \\*
    &                   & \FeII\  &       &  10          & <13.57        & \\
 25 & SBS~1108+560      & \HI\    &   778 &    \nodata   &    \nodata    & No \lya\ fit possible \\*
    &                   & \CI\    &       &  10          & <13.03        & \\*
    &                   & \CII\   &       &              & <15.53        & Blended with Ly-series at $z=0.4634$ \\*
    &                   & \CIV\   &   778 &  36.2\pm 5.4 &  13.94\pm0.04 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &  10          & <13.02        & \\*
    &                   & \SiIII\ &   794 &  10.0\pm 0.0 &  13.40\pm0.74 & \\*
    &                   & \SiIV\  &   778 &  42.8\pm11.4 &  12.86\pm0.09 & Simultaneous fit to doublet, $cz$ fixed \\*
    &                   & \NV\    &       &  40          & <13.93        & \\*
    &                   & \FeII\  &       &  10          & <13.57        & \\
 26 & SBS~1122+594      & \HI\    &  1221 &  44.8\pm 5.2 &  15.94\pm0.47 & BLA; Voigt profile fit to \lya\ \\*
    &                   & \CI\    &       &  30          & <13.36        & \\*
    &                   & \CII\   &  1198 &  34.6\pm 7.1 &  13.80\pm0.06 & 1334~\AA\ line only \\*
    &                   & \CIV\   &  1194 &  39.6\pm 1.5 &  14.74\pm0.03 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &  30          & <12.83        & \\*
    &                   & \SiIII\ &  1215 &  46.3\pm 3.3 &  13.39\pm0.03 & \\*
    &                   & \SiIV\  &  1208 &  39.9\pm 3.6 &  13.54\pm0.03 & Simultaneous fit to doublet \\*
    &                   & \OI\    &       &  30          & <13.88        & \\*
    &                   & \NV\    &       &  45          & <13.64        & \\*
    &                   & \FeII\  &       &  30          & <13.82        & \\
 27 & VII~Zw~244        & \HI\    &   715 &  35.4\pm 3.5 &  15.22\pm0.28 & Voigt profile fit to \lya\ \\*
    &                   & \CI\    &       &  15          & <13.10        & \\*
    &                   & \CII\   &   718 &  14.7\pm 3.0 &  13.53\pm0.04 & \\*
    &                   & \CIV\   &   708 &  23.1\pm 3.7 &  13.62\pm0.04 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &   708 &  29.3\pm 9.6 &  12.31\pm0.09 & 1260~\AA\ line only \\*
    &                   & \SiIII\ &   719 &  20.5\pm 1.4 &  13.17\pm0.03 & \\*
    &                   & \SiIV\  &   715 &  19.2\pm 2.5 &  12.89\pm0.03 & Simultaneous fit to doublet \\*
    &                   & \NV\    &       &  35          & <13.03        & \\*
    &                   & \FeII\  &       &  15          & <13.50        & \\
101 & 3C~273            & \HI\    &  1019 &  35.9\pm 0.4 &  14.28\pm0.01 & CoG \\*
    &                   & \OVI\   &  1007 &  28.0\pm 1.0 &  13.35\pm0.08 & \citet{savage14} \\
102 & 3C~273            & \HI\    &  1585 &  19.9\pm 0.6 &  15.49\pm0.05 & CoG \\*
    &                   & \CII\   &  1593 &  22.8\pm 3.8 &  12.98\pm0.08 & 1334~\AA\ line only \\*
    &                   & \CIII\  &       &              & <13.06        & \citet{tilton12} \\*
    &                   & \CIV\   &       &              & <12.50        & \citet{tripp02} \\*
    &                   & \SiII\  &  1575 &  18.5\pm 4.5 &  11.87\pm0.08 & 1260~\AA\ line only \\*
    &                   & \SiIII\ &  1588 &   6.0\pm 2.9 &  12.09\pm0.05 & \\*
    &                   & \SiIV\  &       &  20          & <12.23        & \\*
    &                   & \OI\    &       &  20          & <13.00        & \\*
    &                   & \OVI\   &       &              & <12.90        & \citet{tilton12} \\*
    &                   & \NV\    &       &  20          & <12.47        & \\*
    &                   & \FeII\  &       &  20          & <13.17        & \\*
    &                   & \FeIII\ &       &              & <13.21        & \citet{tilton12} \\
103 & 3C~351            & \HI\    &  3465 &  41.1\pm 4.8 &  13.47\pm0.05 & BLA; Voigt profile fit to \lya \\
104 & 3C~351            & \HI\    &  3597 &  39.2\pm 3.0 &  13.66\pm0.03 & Voigt profile fit to \lya \\
105 & H~1821+643        & \HI\    & 36139 &  26.5\pm 6.9 &  12.42\pm0.07 & Simultaneous fit to \lya+Ly$\beta$ \\
106 & H~1821+643        & \HI\    & 36307 &  25.0\pm 4.2 &  13.55\pm0.16 & Simultaneous fit to \lya+Ly$\beta$ \\
107 & H~1821+643        & \HI\    & 36339 &  46.5\pm 1.9 &  14.12\pm0.03 & BLA; simultaneous fit to \lya+Ly$\beta$ \\
108 & H~1821+643        & \HI\    & 36439 &  74.0\pm10.9 &  13.60\pm0.10 & BLA; simultaneous fit to \lya+Ly$\beta$ \\*
    &                   & \OVI\   & 36415 &  50.3\pm 8.6 &  13.68\pm0.13 & 1032~\AA\ line only \\
109 & H~1821+643        & \HI\    & 36631 &  37.4\pm 2.7 &  13.09\pm0.02 & Simultaneous fit to \lya+Ly$\beta$ \\
110 & Mrk~335           & \HI\    &  1961 &  30.2\pm 1.3 &  13.81\pm0.01 & Voigt profile fit to \lya\ \\
111 & Mrk~335           & \HI\    &  2281 &  34.7\pm 4.3 &  13.18\pm0.04 & Voigt profile fit to \lya\ \\*
    &                   & \OVI\   &       &              & <13.20        & \citet{tilton12} \\
112 & Mrk~876           & \HI\    &   923 &  48.1\pm 4.2 &  13.90\pm0.10 & BLA; Voigt profile fit to \lya\ \\*
    &                   & \OVI\   &   932 &  25.0\pm 6.0 &  13.55\pm0.08 & \citet{tilton12} \\
113 & Mrk~876           & \HI\    &   978 &  28.1\pm 3.3 &  13.55\pm0.60 & Voigt profile fit to \lya\ \\
114 & PG~0953+414       & \HI\    & 42512 &  15.0\pm 4.5 &  12.66\pm0.07 & Simultaneous fit to \lya-Ly$\gamma$ \\
115 & PG~0953+414       & \HI\    & 42664 &  27.6\pm 1.5 &  13.53\pm0.02 & Simultaneous fit to \lya-Ly$\gamma$ \\*
    &                   & \CII\   &       &  10          & <12.64        & \\*
    &                   & \CIII\  & 42635 &  43.9\pm22.4 &  12.86\pm0.18 & \\*
    &                   & \CIV\   & 42654 &   9.9\pm 6.1 &  12.97\pm0.11 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &  10          & <11.68        & \\*
    &                   & \SiIII\ &       &  25          & <11.77        & \\*
    &                   & \SiIV\  &       &  25          & <12.53        & \\*
    &                   & \OI\    &       &  10          & <13.17        & \\*
    &                   & \OVI\   & 42676 &  21.1\pm 1.4 &  14.03\pm0.02 & Simultaneous fit to doublet \\*
    &                   & \NV\    & 42663 &  12.9\pm 7.0 &  12.76\pm0.13 & 1238~\AA\ line only \\*
    &                   & \FeII\  &       &  10          & <13.11        & \\*
    &                   & \FeIII\ &       &  10          & <13.26        & \\
116 & PG~0953+414       & \HI\    & 42759 &  30.2\pm 2.2 &  13.42\pm0.02 & Simultaneous fit to \lya-Ly$\gamma$ \\*
    &                   & \CIII\  & 42767 &  12.6\pm 6.1 &  12.90\pm0.11 & \\*
    &                   & \SiIII\ & 42769 &  46.3\pm19.5 &  11.97\pm0.23 & \\*
    &                   & \OVI\   & 42763 &  25.4\pm 4.5 &  13.52\pm0.04 & Simultaneous fit to doublet \\
117 & PG~0953+414       & \HI\    & 42907 &  53.1\pm 6.1 &  13.15\pm0.04 & BLA; simultaneous fit to \lya-Ly$\gamma$ \\*
    &                   & \OVI\   & 42873 &  11.8\pm 6.8 &  13.08\pm0.09 & Simultaneous fit to doublet \\
118 & PG~1116+215       & \HI\    & 17614 &  22.0\pm 3.0 &  12.73\pm0.07 & \citet{savage14} \\
119 & PG~1116+215       & \HI\    & 17676 &  33.0\pm 2.0 &  13.57\pm0.01 & \citet{savage14} \\*
    &                   & \OVI\   & 17679 &  27.0\pm16.0 &  13.49\pm0.05 & \citet{savage14} \\
120 & PG~1116+215       & \HI\    & 17786 &  25.0\pm 3.0 &  12.78\pm0.03 & \citet{savage14} \\*
    &                   & \CIV\   & 17761 &  12.0\pm 3.0 &  12.73\pm0.05 & \citet{savage14} \\*
    &                   & \OVI\   & 17762 &   8.0\pm 9.0 &  13.47\pm0.11 & \citet{savage14} \\*
    &                   & \NV\    & 17782 &  20.2\pm 6.2 &  13.11\pm0.09 & 1238~\AA\ line only \\
121 & PG~1116+215       & \HI\    & 18202 &  26.8\pm 3.2 &  13.17\pm0.03 & Voigt profile fit to \lya\ \\
122 & PG~1116+215       & \HI\    & 41522 &  59.8\pm 5.7 &  13.78\pm0.10 & BLA; simultaneous fit to \lya-Ly6 \\
123 & PG~1116+215       & \HI\    & 41522 &  21.7\pm 0.3 &  15.95\pm0.03 & Simultaneous fit to \lya-Ly6 \\*
    &                   & \CII\   & 41522 &   9.6\pm 1.1 &  13.80\pm0.03 & Simultaneous fit to 1036 \& 1334~\AA\ lines \\*
    &                   & \CIII\  & 41515 &  13.0\pm 1.0 &  13.56\pm0.09 & \citet{tilton12} \\*
    &                   & \CIV\   & 41517 &  15.8\pm 4.3 &  13.16\pm0.07 & Simultaneous fit to doublet \\*
    &                   & \SiII\  & 41522 &  22.9\pm 0.9 &  12.63\pm0.01 & Simultaneous fit to 5 available lines \\*
    &                   & \SiIII\ & 41519 &  10.2\pm 0.8 &  12.89\pm0.03 & \\*
    &                   & \SiIV\  & 41514 &   4.4\pm 3.4 &  12.71\pm0.15 & Simultaneous fit to doublet \\*
    &                   & \OI\    &       &  10          & <13.14        & \\*
    &                   & \OVI\   & 41529 &  34.1\pm 2.7 &  13.78\pm0.02 & Simultaneous fit to doublet \\*
    &                   & \NV\    & 41517 &  14.4\pm 3.6 &  12.91\pm0.09 & 1238~\AA\ line only \\*
    &                   & \FeII\  &       &  10          & <13.04        & \\*
    &                   & \FeIII\ &       &  10          & <13.19        & \\
124 & PG~1211+143       & \HI\    &  2114 &  65.2\pm 3.9 &  13.45\pm0.03 & BLA; Voigt profile fit to \lya\ \\*
    &                   & \OVI\   &       &              & <13.87        & Upper limit from intervening line \\
125 & PG~1211+143       & \HI\    & 15170 &   8.3\pm 1.0 &  12.83\pm0.04 & Simultaneous fit to \lya-Ly$\delta$ \\
126 & PG~1211+143       & \HI\    & 15321 &  33.3\pm 1.3 &  15.54\pm0.06 & Simultaneous fit to \lya-Ly$\delta$ \\*
    &                   & \CII\   & 15353 &   6.0\pm 2.0 &  13.15\pm0.10 & \citet{tumlinson05} \\*
    &                   & \CIII\  & 15284 &   8.0\pm 0.0 &  12.99\pm0.05 & \citet{tumlinson05} \\*
    &                   & \CIII\  & 15337 &  20.0\pm 2.5 &  13.92\pm0.08 & \citet{tumlinson05} \\*
    &                   & \CIV\   & 15283 &   8.0\pm 3.0 &  13.02\pm0.08 & \citet{tumlinson05} \\*
    &                   & \CIV\   & 15319 &   9.0\pm 3.5 &  13.08\pm0.13 & \citet{tumlinson05} \\*
    &                   & \CIV\   & 15340 &   6.0\pm 3.5 &  13.75\pm0.59 & \citet{tumlinson05} \\*
    &                   & \CIV\   & 15354 &   5.0\pm 2.5 &  13.43\pm0.22 & \citet{tumlinson05} \\*
    &                   & \SiII\  & 15354 &   5.0\pm 1.0 &  12.25\pm0.05 & \citet{tumlinson05} \\*
    &                   & \SiIII\ & 15342 &  20.0\pm 2.0 &  12.82\pm0.06 & \citet{tumlinson05} \\*
    &                   & \SiIII\ & 15356 &   5.0\pm 0.0 &  12.37\pm0.10 & \citet{tumlinson05} \\*
    &                   & \SiIV\  & 15334 &   7.0\pm 1.0 &  12.49\pm0.07 & \citet{tumlinson05} \\*
    &                   & \SiIV\  & 15353 &   5.0\pm 1.5 &  12.67\pm0.06 & \citet{tumlinson05} \\*
    &                   & \OVI\   & 15341 &  53.0\pm 9.5 &  14.26\pm0.07 & \citet{tumlinson05} \\*
    &                   & \NV\    & 15341 &  15.0\pm 8.0 &  12.98\pm0.17 & \citet{tumlinson05} \\
127 & PG~1211+143       & \HI\    & 15357 & 127.8\pm 9.0 &  14.18\pm0.06 & BLA; simultaneous fit to \lya-Ly$\delta$ \\
128 & PG~1211+143       & \HI\    & 15431 &  32.2\pm 2.5 &  14.17\pm0.05 & Simultaneous fit to \lya-Ly$\delta$ \\
129 & PG~1211+143       & \HI\    & 15574 &  37.5\pm 2.2 &  13.49\pm0.03 & Simultaneous fit to \lya-Ly$\delta$ \\
130 & PG~1211+143       & \HI\    & 19305 &  31.3\pm 0.4 &  15.31\pm0.04 & Simultaneous fit to \lya-Ly$\delta$ \\*
    &                   & \CIII\  & 19277 &   4.0\pm 3.5 &  13.89\pm0.91 & \citet{tumlinson05} \\*
    &                   & \CIII\  & 19310 &  27.0\pm 7.5 &  13.23\pm0.08 & \citet{tumlinson05} \\*
    &                   & \CIV\   & 19328 &  43.7\pm 3.9 &  13.32\pm0.07 & \citet{tilton12} \\*
    &                   & \SiIII\ & 19328 &  38.0\pm 1.0 &  12.22\pm0.04 & \citet{tilton12} \\*
    &                   & \OVI\   & 19356 &  37.0\pm 6.5 &  14.08\pm0.06 & \citet{tumlinson05} \\
131 & PG~1211+143       & \HI\    & 19424 &  28.0\pm 2.4 &  13.77\pm0.04 & Simultaneous fit to \lya-Ly$\delta$ \\*
    &                   & \OVI\   & 19434 &  21.0\pm10.0 &  13.63\pm0.16 & \citet{tumlinson05} \\
132 & PG~1211+143       & \HI\    & 19481 &  30.1\pm10.1 &  13.29\pm0.17 & Simultaneous fit to \lya-Ly$\delta$ \\*
    &                   & \CIII\  & 19474 &  18.0\pm 7.5 &  12.96\pm0.05 & \citet{tumlinson05} \\*
    &                   & \CIV\   & 19466 &  24.0\pm 5.0 &  13.10\pm0.21 & \citet{tilton12} \\*
    &                   & \SiIII\ &       &              & <12.22        & \citet{tilton12} \\
133 & PG~1211+143       & \HI\    & 19557 &  35.6\pm 7.1 &  13.06\pm0.09 & Simultaneous fit to \lya-Ly$\delta$ \\
134 & PG~1216+069       & \HI\    & 23880 &  63.3\pm14.0 &  13.14\pm0.07 & BLA; Voigt profile fit to \lya\ \\
135 & PG~1216+069       & \HI\    & 24059 &  24.7\pm 8.7 &  13.14\pm0.16 & Voigt profile fit to \lya\ \\
136 & PG~1216+069       & \HI\    & 24141 &  42.3\pm 2.8 &  14.15\pm0.02 & BLA; Voigt profile fit to \lya\ \\
137 & PG~1216+069       & \HI\    & 37049 &  25.4\pm 1.5 &  14.57\pm0.05 & Simultaneous fit to \lya+Ly$\beta$ \\*
    &                   & \CII\   &       &  10          & <12.99        & \\*
    &                   & \CIII\  & 37091 &  84.0\pm 2.0 &  13.83\pm0.20 & \citet{tilton12} \\*
    &                   & \CIV\   & 37055 &  11.6\pm 1.7 &  13.95\pm0.08 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &  10          & <11.89        & \\*
    &                   & \SiIII\ & 37057 &  20.4\pm 4.2 &  12.46\pm0.09 & \\*
    &                   & \SiIV\  & 37047 &  26.7\pm10.9 &  12.72\pm0.15 & 1393~\AA\ line only \\*
    &                   & \OI\    &       &  10          & <13.35        & \\*
    &                   & \OVI\   & 37062 &  27.8\pm 4.9 &  14.14\pm0.06 & Simultaneous fit to doublet \\*
    &                   & \NV\    & 37054 &  10.1\pm 3.9 &  13.23\pm0.06 & Simultaneous fit to doublet \\*
    &                   & \FeII\  &       &  10          & <13.28        & \\
138 & PG~1216+069       & \HI\    & 37138 &  24.9\pm 1.4 &  14.76\pm0.05 & Simultaneous fit to \lya+Ly$\beta$ \\*
    &                   & \CII\   &       &  10          & <12.99        & \\*
    &                   & \CIII\  &       &              & <13.83        & Upper limit from intervening line \\*
    &                   & \CIV\   & 37137 &  14.7\pm 2.2 &  13.78\pm0.05 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &  10          & <11.89        & \\*
    &                   & \SiIII\ & 37141 &   6.1\pm 3.7 &  12.35\pm0.11 & \\*
    &                   & \SiIV\  & 37134 &  10.5\pm 7.3 &  12.59\pm0.14 & 1393~\AA\ line only \\*
    &                   & \OI\    &       &  10          & <13.35        & \\*
    &                   & \OVI\   & 37143 &  33.9\pm 6.4 &  14.12\pm0.06 & Simultaneous fit to doublet \\*
    &                   & \NV\    & 37134 &  22.5\pm10.5 &  13.01\pm0.12 & Simultaneous fit to doublet \\*
    &                   & \FeII\  &       &  10          & <13.28        & \\
139 & PG~1216+069       & \HI\    & 37363 &  38.7\pm 1.6 &  14.68\pm0.03 & Simultaneous fit to \lya+Ly$\beta$ \\*
    &                   & \CIV\   & 37373 &  10.0\pm 0.0 &  13.26\pm0.12 & Simultaneous fit to doublet \\*
    &                   & \SiIII\ & 37371 &  11.2\pm 4.8 &  12.20\pm0.07 & \\*
    &                   & \OVI\   & 37370 &  33.9\pm32.4 &  13.51\pm0.48 & Simultaneous fit to doublet \\*
140 & PG~1216+069       & \HI\    & 37455 &  21.8\pm 2.0 &  14.05\pm0.05 & Simultaneous fit to \lya+Ly$\beta$ \\*
    &                   & \CIV\   & 37432 &  31.4\pm 8.0 &  13.52\pm0.07 & Simultaneous fit to doublet \\*
    &                   & \OVI\   & 37443 &  34.1\pm11.8 &  13.97\pm0.17 & Simultaneous fit to doublet \\*
141 & PG~1259+593       & \HI\    &   702 &  38.4\pm 0.9 &  13.71\pm0.01 & Voigt profile fit to \lya\ \\*
    &                   & \OVI\   &   657 &  75.0\pm 0.0 &  13.61\pm0.07 & 1032~\AA\ line only \\
142 & PG~1259+593       & \HI\    & 13825 &  31.9\pm 1.0 &  15.45\pm0.04 & Simultaneous fit to \lya-Ly5 \\*
    &                   & \CI\    &       &  15          & <12.79        & \\*
    &                   & \CII\   &       &              & <14.35        & Upper limit from intervening line \\*
    &                   & \CIII\  & 13821 &  29.3\pm 2.4 &  13.85\pm0.04 & \\*
    &                   & \CIV\   & 13839 &  27.6\pm 3.5 &  13.65\pm0.04 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &  15          & <11.92        & \\*
    &                   & \SiIII\ & 13821 &  29.7\pm 1.9 &  12.87\pm0.02 & \\*
    &                   & \SiIV\  & 13830 &  37.3\pm 6.4 &  12.67\pm0.05 & Simultaneous fit to doublet \\*
    &                   & \OI\    &       &  15          & <13.22        & \\*
    &                   & \OVI\   & 13830 &  40.0\pm12.9 &  13.94\pm0.12 & 1032~\AA\ line only \\*
    &                   & \NV\    &       &  15          & <13.21        & \\*
    &                   & \FeII\  &       &  15          & <13.12        & \\*
    &                   & \FeIII\ &       &  15          & <13.36        & \\
143 & PG~1259+593       & \HI\    & 13914 &  34.7\pm 3.4 &  14.60\pm0.05 & Simultaneous fit to \lya-Ly5 \\*
    &                   & \CI\    &       &  15          & <12.79        & \\*
    &                   & \CII\   &       &              & <14.35        & Upper limit from intervening line \\*
    &                   & \CIII\  & 13905 &  18.5\pm 2.9 &  13.45\pm0.05 & \\*
    &                   & \CIV\   & 13921 &  16.0\pm 5.4 &  13.49\pm0.10 & 1550~\AA\ line only \\*
    &                   & \SiII\  &       &  15          & <11.92        & \\*
%    &                   & \SiIII\ & 13942 &  39.8\pm 3.1 &  12.78\pm0.04 & \\*
    &                   & \SiIII\ & 13942 &  39.8\pm 3.1 & <12.78        & Upper limit from intervening line \\*
    &                   & \SiIV\  &       &              & <12.67        & \\*
    &                   & \OI\    &       &  15          & <13.22        & \\*
    &                   & \OVI\   & 13899 &  16.7\pm 8.3 &  13.71\pm0.15 & 1032~\AA\ line only \\*
    &                   & \NV\    &       &  15          & <13.21        & \\*
    &                   & \FeII\  &       &  15          & <13.12        & \\*
    &                   & \FeIII\ &       &  15          & <13.36        & \\
144 & PG~1259+593       & \HI\    & 14014 &  34.6\pm 3.1 &  13.58\pm0.03 & Simultaneous fit to \lya-Ly5 \\
145 & PHL~1811          & \HI\    & 15418 &  72.8\pm 5.1 &  13.65\pm0.03 & BLA; Voigt profile fit to \lya\ \\*
146 & PHL~1811          & \HI\    & 15444 &  35.9\pm 2.0 &  13.60\pm0.02 & Voigt profile fit to \lya\ \\*
    &                   & \CIV\   & 15479 &  17.4\pm 7.5 &  12.96\pm0.16 & 1548~\AA\ line only \\
147 & PHL~1811          & \HI\    & 21998 &  24.2\pm 3.9 &  14.42\pm0.15 & Simultaneous fit to \lya-Ly$\gamma$ \\
148 & PHL~1811          & \HI\    & 22042 &  22.6\pm 2.8 &  14.68\pm0.09 & Simultaneous fit to \lya-Ly$\gamma$ \\*
    &                   & \SiIII\ & 22028 &  78.1\pm 8.2 &  12.73\pm0.10 & \\*
    &                   & \OVI\   &       &              & <13.03        & \citet{tilton12} \\
149 & PHL~1811          & \HI\    & 23313 &  23.1\pm 0.5 &  15.40\pm0.07 & Simultaneous fit to \lya-Ly$\gamma$ \\*
    &                   & \CI\    &       &  20          & <12.79        & \\*
    &                   & \CII\   &       &              & <13.22        & Upper limit from intervening line \\*
    &                   & \CIII\  & 23315 &  22.0\pm 2.0 &  13.55\pm0.05 & \citet{tilton12} \\*
    &                   & \CIV\   &       &  25          & <12.88        & \\*
    &                   & \SiII\  & 23303 &  18.6\pm 4.2 &  12.31\pm0.08 & 1260~\AA\ line only \\*
    &                   & \SiIII\ & 23310 &  18.9\pm 2.7 &  12.52\pm0.05 & \\*
    &                   & \SiIV\  &       &  20          & <12.27        & \\*
    &                   & \OVI\   &       &              & <13.12        & \citet{tilton12} \\*
    &                   & \FeII\  &       &  20          & <13.08        & \\*
    &                   & \FeIII\ &       &  20          & <14.23        & \\
150 & PHL~1811          & \HI\    & 23652 &  13.8\pm 1.8 &  15.04\pm0.29 & Simultaneous fit to \lya-Ly$\beta$ \\*
    &                   & \OVI\   &       &              & <13.12        & \citet{tilton12} \\
151 & PHL~1811          & \HI\    & 23710 &  25.0\pm 1.9 &  14.65\pm0.06 & Simultaneous fit to \lya-Ly$\beta$ \\
152 & PHL~1811          & \HI\    & 24226 &  30.2\pm 0.5 &  18.08\pm0.04 & Simultaneous fit to \lya-Ly6 \\*
    &                   & \CI\    &       &  17          & <13.45        & \\*
    &                   & \CII\   & 24260 &  16.6\pm 0.5 &  14.13\pm0.01 & Simultaneous fit to 1036 \& 1334~\AA\ lines \\*
    &                   & \CIII\  & 24224 &  41.0\pm 2.0 &  14.06\pm0.06 & \citet{tilton12} \\*
    &                   & \CIV\   & 24207 &  17.0\pm 3.2 &  13.40\pm0.04 & Simultaneous fit to doublet \\*
    &                   & \CIV\   & 24261 &  12.2\pm 1.1 &  13.90\pm0.04 & Simultaneous fit to doublet \\*
    &                   & \SiII\  & 24259 &   8.4\pm 0.3 &  13.82\pm0.03 & Simultaneous fit to 5 available lines \\*
    &                   & \SiIV\  & 24258 &  12.4\pm 0.8 &  13.38\pm0.02 & Simultaneous fit to doublet \\*
    &                   & \OI\    & 24256 &  23.3\pm 0.9 &  14.45\pm0.02 & \\*
    &                   & \OVI\   &       &              & <13.88        & \citet{tilton12} \\*
    &                   & \NV\    &       &  29          & <12.87        & \\*
    &                   & \FeII\  & 24252 &  12.5\pm 2.0 &  13.68\pm0.03 & Simultaneous fit to 4 available lines \\
153 & PHL~1811          & \HI\    & 39658 &  31.5\pm 0.4 &  14.61\pm0.01 & Simultaneous fit to \lya-Ly$\delta$ \\*
    &                   & \CII\   &       &  15          & <12.87        & \\*
    &                   & \CIII\  & 39639 &  16.6\pm12.2 &  12.72\pm0.20 & \\*
    &                   & \CIV\   & 39662 &  26.8\pm 8.9 &  13.07\pm0.10 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &  15          & <11.71        & \\*
    &                   & \SiIII\ &       &  15          & <11.68        & \\*
    &                   & \SiIV\  &       &  25          & <12.45        & \\*
    &                   & \OI\    &       &  15          & <13.88        & \\*
    &                   & \OVI\   & 39695 &  52.7\pm 4.2 &  13.88\pm0.02 & Simultaneous fit to doublet \\*
    &                   & \FeII\  &       &  15          & <13.10        & \\*
    &                   & \FeIII\ &       &  15          & <13.17        & \\
154 & PHL~1811          & \HI\    & 39795 &  60.9\pm 8.0 &  13.19\pm0.04 & BLA; simultaneous fit to \lya-Ly$\delta$ \\*
    &                   & \OVI\   & 39826 &  22.4\pm 3.6 &  13.59\pm0.04 & Simultaneous fit to doublet \\*
155 & PHL~1811          & \OVI\   & 39930 &  33.2\pm 4.6 &  13.61\pm0.04 & No associated \HI; simultaneous fit to doublet \\
156 & PHL~1811          & \HI\    & 52914 &  41.7\pm 0.9 &  14.22\pm0.03 & BLA; simultaneous fit to \lya-Ly5 \\*
    &                   & \OVI\   & 52922 &  18.1\pm 2.2 &  14.11\pm0.03 & 1038~\AA\ line only \\
157 & PHL~1811          & \HI\    & 52933 &  17.8\pm 1.3 &  14.84\pm0.04 & Simultaneous fit to \lya-Ly5 \\*
    &                   & \CII\   &       &  10          & <12.89        & \\*
    &                   & \CIII\  & 52938 &  11.2\pm 3.7 &  13.29\pm0.08 & \\*
    &                   & \SiII\  &       &  10          & <11.69        & \\*
    &                   & \SiIII\ & 52935 &  19.5\pm 3.5 &  12.14\pm0.07 & \\*
    &                   & \SiIV\  & 52945 &   8.9\pm11.5 &  12.36\pm0.14 & 1393~\AA\ line only, marginal detection \\*
    &                   & \OI\    &       &  10          & <13.17        & \\*
    &                   & \OVI\   &       &              & <14.11        & \\*
    &                   & \NV\    &       &  20          & <12.55        & \\*
    &                   & \FeII\  &       &  10          & <12.89        & \\*
    &                   & \FeIII\ &       &  10          & <13.15        & \\
158 & PKS~0312--770     & \HI\    & 17824 &  35.0\pm 2.0 &  13.53\pm0.03 & \citet{tilton12} \\*
    &                   & \SiIII\ & 17824 &  21.0\pm 6.0 &  12.07\pm0.15 & \\
159 & PKS~0312--770     & \HI\    & 35466 &  32.0\pm 2.0 &  14.17\pm0.04 & \citet{tilton12} \\
160 & PKS~0312--770     & \HI\    & 35813 &  41.0\pm 2.0 &  13.79\pm0.02 & BLA; \citet{tilton12} \\
161 & PKS~0405--123     & \HI\    & 28947 &  29.0\pm 1.0 &  14.58\pm0.02 & \citet{savage14} \\
162 & PKS~0405--123     & \HI\    & 28958 &  69.0\pm 3.0 &  13.93\pm0.04 & BLA; \citet{savage14} \\*
    &                   & \OVI\   & 28955 &  23.0\pm 6.0 &  13.70\pm0.07 & \citet{savage14} \\
163 & PKS~0405--123     & \HI\    & 45617 &  24.9\pm 0.6 &  13.37\pm0.01 & Voigt profile fit to \lya\ \\*
    &                   & \OVI\   & 45599 &  18.5\pm 5.1 &  12.96\pm0.06 & 1032~\AA\ line only \\
164 & PKS~0405--123     & \HI\    & 45783 &  13.0\pm 3.0 &  12.48\pm0.06 & Voigt profile fit to \lya\ \\*
    &                   & \OVI\   &       &  13          & <12.78        & \\
165 & PKS~0405--123     & \HI\    & 45871 &  47.6\pm 0.8 &  13.72\pm0.01 & BLA; Voigt profile fit to \lya\ \\*
    &                   & \OVI\   &       &  48          & <13.02        & \\
166 & PKS~0405--123     & \OVI\   & 49780 &  56.0\pm 2.0 &  13.85\pm0.01 & No associated \HI; \citet{savage14} \\
167 & PKS~0405--123     & \HI\    & 49910 &  54.0\pm13.0 &  13.11\pm0.16 & BLA; \citet{savage14} \\*
168 & PKS~0405--123     & \HI\    & 49946 &  12.0\pm 1.0 &  13.35\pm0.05 & \citet{savage14} \\*
    &                   & \CIII\  & 49943 &  39.7\pm 2.0 &  13.51\pm0.01 & \\*
    &                   & \SiIV\  & 49952 &  14.6\pm 5.3 &  12.31\pm0.08 & Simultaneous fit to doublet \\*
    &                   & \OVI\   & 49947 &  29.0\pm 2.0 &  13.89\pm0.04 & \citet{savage14} \\*
    &                   & \NV\    & 49775 &  28.8\pm 3.6 &  13.17\pm0.06 & 1238~\AA\ line only \\
169 & PKS~0405--123     & \HI\    & 50001 &  27.0\pm 5.0 &  13.56\pm0.08 & \citet{savage14} \\*
    &                   & \OVI\   &       &              & <14.23        & \citet{savage14} \\*
    &                   & \NV\    & 50005 &  24.1\pm 5.6 &  13.12\pm0.09 & 1238~\AA\ line only \\
170 & PKS~0405--123     & \HI\    & 50059 &  16.0\pm 1.0 &  15.41\pm0.06 & \citet{savage14} \\*
    &                   & \CII\   & 50054 &  10.7\pm 1.6 &  13.53\pm0.02 & Simultaneous fit to 1036 \& 1334~\AA\ lines \\*
    &                   & \CIII\  & 50072 &  35.3\pm 1.4 &  14.42\pm0.05 & \\*
    &                   & \SiII\  & 50085 &  41.3\pm 1.6 &  12.90\pm0.02 & Simultaneous fit to 5 available lines \\*
    &                   & \SiIII\ & 50053 &  13.0\pm 1.0 &  12.66\pm0.03 & \\*
    &                   & \SiIV\  &       &              & <13.14        & Upper limit from intervening line \\*
    &                   & \OI\    &       &              & <13.52        & Upper limit from intervening line \\*
    &                   & \OVI\   & 50029 &  38.0\pm 5.0 &  14.23\pm0.07 & \citet{savage14} \\*
    &                   & \NV\    &       &              & <13.12        & \\*
    &                   & \FeII\  &       &              & <13.10        & \\*
    &                   & \FeIII\ &       &   5.0\pm 0.0 & <13.07        & \\
171 & PKS~0405--123     & \HI\    & 50104 &  26.0\pm 1.0 &  16.45\pm0.02 & \citet{savage14} \\*
    &                   & \CII\   & 50100 &  13.9\pm 0.6 &  14.26\pm0.02 & Simultaneous fit to 1036 \& 1334~\AA\ lines \\*
    &                   & \CIII\  &       &              & <14.42        & \\*
    &                   & \SiII\  & 50112 &   8.9\pm 0.5 &  13.11\pm0.02 & Simultaneous fit to 5 available lines \\*
    &                   & \SiIII\ & 50100 &  22.5\pm 0.6 &  13.29\pm0.01 & \\*
    &                   & \SiIV\  & 50105 &  26.8\pm 1.5 &  13.14\pm0.02 & Simultaneous fit to doublet \\*
    &                   & \OI\    &       &              & <13.52        & Upper limit from intervening line \\*
    &                   & \OVI\   & 50105 &  39.0\pm 2.0 &  14.45\pm0.03 & \citet{savage14} \\*
    &                   & \NV\    & 50092 &  40.7\pm 1.8 &  13.86\pm0.02 & 1238~\AA\ line only \\*
    &                   & \FeII\  &       &              & <13.10        & \\*
    &                   & \FeIII\ & 50098 &   5.0\pm 0.0 &  13.07\pm0.07 & \\
172 & PKS~0405--123     & \HI\    & 50158 &  41.0\pm 3.0 &  13.90\pm0.08 & BLA; \citet{savage14} \\
173 & PKS~1302--102     & \HI\    &  3455 &  30.7\pm 3.5 &  13.30\pm0.05 & Voigt profile fit to \lya\ \\
174 & PKS~1302--102     & \HI\    & 12573 &  19.2\pm 3.8 &  13.02\pm0.05 & Simultaneous fit to \lya-Ly$\gamma$ \\
175 & PKS~1302--102     & \HI\    & 12655 &  18.8\pm 1.3 &  14.91\pm0.08 & Simultaneous fit to \lya-Ly$\gamma$ \\*
    &                   & \CI\    &       &  10          & <12.95        & \\*
    &                   & \CII\   & 12652 &  13.0\pm 8.3 &  13.00\pm0.17 & 1334~\AA\ line only \\*
    &                   & \CIII\  & 12655 &  22.6\pm 4.3 &  13.54\pm0.08 & \citet{tilton12} \\*
    &                   & \CIV\   & 12662 &  39.8\pm 9.3 &  13.39\pm0.07 & Simultaneous fit to doublet \\*
    &                   & \SiII\  & 12649 &  22.4\pm14.1 &  12.03\pm0.04 & 1260~\AA\ line only \\*
    &                   & \SiIII\ & 12655 &   9.6\pm 3.2 &  12.41\pm0.06 & \\*
    &                   & \SiIV\  &       &              & <12.57        & Upper limit from intervening line \\*
    &                   & \OI\    &       &  10          & <13.26        & \\*
    &                   & \OVI\   & 12619 &  26.7\pm13.6 &  13.83\pm0.16 & 1032~\AA\ line only \\*
    &                   & \NV\    &       &  40          & <13.19        & \\*
    &                   & \FeII\  &       &  10          & <13.33        & \\*
    &                   & \FeIII\ &       &  10          & <13.37        & \\
176 & PKS~1302--102     & \HI\    & 12703 &  29.1\pm 6.2 &  13.74\pm0.16 & Simultaneous fit to \lya-Ly$\gamma$ \\*
    &                   & \OVI\   & 12694 &  24.0\pm 5.3 &  14.30\pm0.08 & 1032~\AA\ line only \\
177 & PKS~1302--102     & \HI\    & 28179 &  26.4\pm 2.4 &  15.04\pm0.20 & Simultaneous fit to \lya-Ly12\\*
178 & PKS~1302--102     & \HI\    & 28439 &  28.9\pm 0.8 &  17.11\pm0.03 & Simultaneous fit to \lya-Ly12\\*
    &                   & \CII\   & 28469 &  42.3\pm 6.6 &  13.64\pm0.08 & 1334~\AA\ line only \\*
    &                   & \CIII\  & 28418 &  29.7\pm 8.2 &  13.68\pm0.10 & \citet{tilton12} \\*
    &                   & \CIII\  & 28469 &  11.6\pm 8.7 &  13.22\pm0.23 & \citet{tilton12} \\*
    &                   & \CIV\   &       &  50          & <13.13        & \\*
    &                   & \SiII\  & 28442 &  37.3\pm 7.9 &  12.54\pm0.11 & 1260~\AA\ line only \\*
    &                   & \SiIII\ & 28429 &  22.9\pm 3.2 &  12.84\pm0.05 & \\*
    &                   & \SiIII\ & 28479 &  16.4\pm 4.7 &  12.46\pm0.10 & \\*
    &                   & \SiIV\  &       &              & <12.36        & \citet{tilton12} \\*
    &                   & \OI\    &       &  10          & <13.25        & \\*
    &                   & \OVI\   & 28439 &  61.6\pm17.8 &  13.85\pm0.16 & \citet{tilton12} \\*
    &                   & \NV\    &       &  60          & <13.10        & \\*
    &                   & \FeII\  &       &  10          & <13.08        & \\*
    &                   & \FeIII\ &       &  10          & <13.33        & \\
179 & PKS~2155--304     & \HI\    & 16965 &  52.3\pm 0.9 &  14.34\pm0.01 & BLA; Voigt profile fit to \lya\ \\
180 & PKS~2155--304     & \HI\    & 17113 &  67.9\pm 1.7 &  14.08\pm0.01 & BLA; Voigt profile fit to \lya\ \\*
    &                   & \OVI\   & 17149 &  24.3\pm 7.1 &  13.60\pm0.09 & 1032~\AA\ line only \\
181 & PKS~2155--304     & \HI\    & 17340 &  13.9\pm 5.8 &  12.47\pm0.08 & Voigt profile fit to \lya\ \\
182 & PKS~2155--304     & \HI\    & 31635 &  47.1\pm 2.3 &  13.98\pm0.03 & BLA; Voigt profile fit to \lya\ \\*
    &                   & \OVI\   &       &  47          & <13.50        & \\
183 & PKS~2155--304     & \HI\    & 31697 &  21.6\pm 4.4 &  13.33\pm0.15 & Voigt profile fit to \lya\ \\*
    &                   & \OVI\   &       &  22          & <13.35        & \\
184 & PKS~2155--304     & \HI\    & 31754 &  43.2\pm 8.6 &  13.28\pm0.12 & BLA; Voigt profile fit to \lya\ \\*
    &                   & \OVI\   &       &  43          & <13.48        & \\
185 & Q~1230+0115       & \HI\    &  1497 &  24.4\pm 0.7 &  13.68\pm0.01 & Voigt profile fit to \lya\ \\
186 & Q~1230+0115       & \HI\    & 23294 &  35.5\pm 0.9 &  14.50\pm0.03 & Voigt profile fit to \lya\ \\*
    &                   & \CIV\   & 23263 &  29.1\pm 6.1 &  13.80\pm0.13 & Simultaneous fit to doublet \\*
    &                   & \CIV\   & 23307 &  22.1\pm 2.8 &  13.91\pm0.11 & Simultaneous fit to doublet \\*
    &                   & \SiIV\  & 23302 &   5.0\pm 0.0 &  12.05\pm0.10 & Simultaneous fit to doublet, marginal \\
187 & Q~1230+0115       & \HI\    & 23404 &  25.6\pm 1.0 &  14.77\pm0.08 & Voigt profile fit to \lya\ \\*
    &                   & \CI\    &       &  10          & <12.93        & \\*
    &                   & \CII\   &       &  10          & <12.56        & \\*
    &                   & \CIII\  & 23396 &  26.5\pm19.2 &  14.11\pm0.40 & \citet{tilton12} \\*
    &                   & \CIV\   & 23405 &  25.1\pm 0.8 &  14.18\pm0.01 & Simultaneous fit to doublet \\*
    &                   & \SiII\  &       &  10          & <12.20        & \\*
    &                   & \SiIII\ & 23405 &  18.1\pm 2.3 &  12.34\pm0.05 & \\*
    &                   & \SiIV\  & 23403 &  12.4\pm 2.9 &  12.47\pm0.05 & Simultaneous fit to doublet \\*
    &                   & \OI\    &       &  10          & <13.30        & \\*
    &                   & \NV\    &       &  16.2\pm 2.8 &  13.35\pm0.06 & 1242~\AA\ line only \\*
    &                   & \FeII\  &       &  10          & <12.80        & \\*
    &                   & \FeIII\ &       &  10          & <13.35        & \\
\enddata

\end{deluxetable*}

